Embedding Large PQC KEMs in IKEv2

Post-quantum key encapsulation mechanisms carry public keys far larger than the established VPN handshake protocol IKEv2 was designed for. At the same time, its initial exchange comprising the public keys cannot be fragmented. In response, the IETF discusses a range of protocol adjustments, yet these proposals have never been compared in terms of their performance and stability under identical conditions. We systematically screened the IETF document corpus for such proposals, added three of our own (one using forward error correction and two using IKEv2 with QUIC, namely QUIKE and QUIKE with a composite key exchange), identified two specification gaps in existing acknowledgment drafts, and implemented all eight on the same open-source codebase. Measurements across different bandwidths, latencies, and packet loss rates, and with ML-KEM, FrodoKEM, and Classic McEliece, total 126 500 handshakes in 1296 different configurations and show that no mechanism fully compensates for the effect of the key size on performance. For Classic McEliece, no approach handles challenging conditions acceptably. The approaches either congest the link or take up to nearly two minutes per handshake on average. For ML-KEM and FrodoKEM, there are two ways forward: building on already standardized extensions or delegating the transport. The former requires the larger implementation change and needs further optimization, such as acknowledgment mechanisms or error-correcting codes, but grants continuity and compatibility. The latter can use a composite key exchange to avoid these drawbacks and achieve a faster, more resilient handshake and leaner implementation, with QUIKE-composite offering the best overall performance.

==> images/flow-styles.tex <==
% Shared styles for the message-flow figures: ikev2, intermediate, quike and
% quike_composite. Included both when a figure is compiled standalone and when
% main.tex pulls it in with \includestandalone, hence the \imagedir default in
% each figure.
\usetikzlibrary{positioning, arrows, arrows.meta, calc, shadows}

\tikzset{
	node distance=0.5mm and 2mm,
	%
	angle/.style={shading angle=45},
	box/.style={draw=black, line width=1, minimum width=160, minimum
		height=60, align=center, angle, drop shadow},
	component/.style={rectangle, draw=gray, fill=gray, line width=1.5},
	%
	blue_box/.style={top color=blue!35, bottom color=blue, box},
	red_box/.style={top color=red!35, bottom color=red, box},
	green_box/.style={top color=green!35, bottom color=green, box},
	gray_box/.style={top color=gray!35, bottom color=gray, box},
	%
	arrow/.style={draw=blue, line width=3, -stealth},
	% a peer's vertical timeline: the arrow stroke without its tip
	lifeline/.style={arrow, -},
	dma/.style={draw=blue, fill=blue, line width=3,
		-{Latex[length=6mm, width=6mm]}},
	avst/.style={draw=black, line width=3, -{Latex[length=6mm, width=6mm]}},
	%
	% rotated labels flanking the flow: IKEv2 exchanges left, QUIC levels right
	exchange/.style={green_box, rotate=90, minimum height=50,
		minimum width=110},
	level/.style={gray_box, rotate=90, minimum height=50, minimum width=110},
}

